Towards Understanding Human Functional Brain Development with Explainable Artificial Intelligence: Challenges and Perspectives

The last decades have seen significant advancements in non-invasive neuroimaging technologies that have been increasingly adopted to examine human brain development. However, these improvements have not necessarily been followed by more sophisticated data analysis measures that are able to explain the mechanisms underlying functional brain development. For example, the shift from univariate (single area in the brain) to multivariate (multiple areas in brain) analysis paradigms is of significance as it allows investigations into the interactions between different brain regions. However, despite the potential of multivariate analysis to shed light on the interactions between developing brain regions, artificial intelligence (AI) techniques applied render the analysis non-explainable. The purpose of this paper is to understand the extent to which current state-of-the-art AI techniques can inform functional brain development. In addition, a review of which AI techniques are more likely to explain their learning based on the processes of brain development as defined by developmental cognitive neuroscience (DCN) frameworks is also undertaken. This work also proposes that eXplainable AI (XAI) may provide viable methods to investigate functional brain development as hypothesised by DCN frameworks.

==> LaTeX_Figures/BPalgorithm.tex <==
%---------------------------------------------------------------
%---------------------------------------------------------------
%---------------- Backpropagation Algorithm -------------
%---------------------------------------------------------------
%---------------------------------------------------------------
\begin{algorithm}
  \SetAlgoLined
  \KwResult{Updated weights of the DNN}
  initialisation\;
  \For{d in data}{
    \Begin(Forward Pass){
     Starting from the input layer, use eq.~\ref{} to do
     a forward pass through the network, and predict the output\;
     Compute the error between the predicted and the true output\;
    }
    \Begin(Backward Pass){
      \While{error > tolerance}{
        \For{layer in layers}{
        Compute the derivatives of the error function with respect
        to the output layer activities\;
        }
         Updates the weights.
      }
     }
  }
  \caption{Backpropagation Algorithm}
  \label{algo:BP}
\end{algorithm}
%---------------------------------------------------------------
%---------------------------------------------------------------

==> LaTeX_Figures/FCM_table.tex <==
\scalebox{1.1}{
\begin{tabular}{l l l l l l l } % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
     \rowcolor{blue!15}&\textbf{Ch1} & \textbf{Ch2} & \textbf{Ch3}&\textbf{Ch4}  & \textbf{Ch5} & \textbf{Ch6}\\      
     \hline             %Ch1	Ch2	Ch3		Ch4		Ch5	CH6	Ch7
      \rowcolor{blue!5}\textbf{Ch1} &  		&0.5 	& 			&0.25 		& 		&			 	\\ 
      \rowcolor{blue!15}\textbf{Ch2} &  		& 		& -0.1		& -1		& 		&				\\ 
      \rowcolor{blue!5}\textbf{Ch3} &  		&  		& 			& 			& 0.7	&0.4			\\ 
      \rowcolor{blue!15}\textbf{Ch4} &  		&0.1 	& 			& 			&0.5	&				\\ 
      \rowcolor{blue!5}\textbf{Ch5} &  		&-0.4	&	 		& 			&		&-0.15			 \\ 
     \rowcolor{blue!15} \textbf{Ch6} &  		& 		& 			& 			& 		&				\\ \hline
\end{tabular}}


==> LaTeX_Figures/MVPA_schematic.tex <==
\tikzstyle{blockgraphics} = [rectangle]
\tikzstyle{block} = [rectangle, rounded corners, draw, text width=11.5cm, text badly centered, minimum height = 1 cm]
\tikzstyle{dotted_block} = [draw=black!30!white, line width=1pt, dash pattern=on 1pt off 4pt on 6pt off 4pt,
            inner ysep=6mm,inner xsep=4mm, rectangle, rounded corners ]
\tikzstyle{myarrows} = [ultra thick,->]
\begin{figure*}[!htbp]
%\centering
%-------------------------------------------------
\scalebox{0.8}{
%trim={<left> <lower> <right> <upper>}
\begin{tikzpicture}[node distance =3.7cm]
% nodes
\node (baby) [anchor=south west,inner sep=0]  {\scalebox{-1}[1]{\includegraphics[scale = 0.4, trim ={1cm 6.3cm 13cm 1cm}, clip]{Figures/Lateral_Back_electrodepositions.jpg}}};
\node (preprocessing) [block, right of = baby, text width = 2.5cm] {Pre-processing};
\node (fselection) [block, right of = preprocessing, text width = 2.5cm] {Feature Selection};
\node (MVPM) [block, right of = fselection, text width = 2.5cm] {Multivariate Matrix (MVM)};
\node (models) [block, right of = MVPM, text width = 3cm] {Machine Learning (ML) Algorithm};
\node (results) [block, right of =models, text width = 2.5cm] {Classification results};
% paths
\draw [myarrows] ([yshift = -1cm]baby.north) |- node[xshift = 1.8cm, yshift = .5cm]{Neuroimaging signals}++(2,1)-| (preprocessing.north);
\draw [myarrows] (preprocessing) -- (fselection);
\draw [myarrows] (fselection) -- (MVPM);
\draw [myarrows] (MVPM) -- (models);
\draw [myarrows] (models) -- (results);
\end{tikzpicture}}
%-------------------------------------------------
\caption{A flowchart of the main stages in a multivariate pattern analysis (MVPA) driven by machine learning (ML) algorithms. The neuroimaging data recorded from a participant's head is preprocessed to remove motion artifacts, and increase the signal to noise ratio. The preprocessed data then undergoes feature selection. For fNIRS data one of the most common statistical features used is the mean of the fNIRS signal, post stimulus presentation, for a given length of time \cite{Emberson_2017}. For EEG signal, averaged event related potentials (ERPs) are most commonly used in DCN studies \cite{Thierry_2005_ERP_infants}. Using the features selected, the multivariate matrix (MVM) is constructed which collates the brain regions activity as read by the neuroimaging technology. The MVM is then fed into a ML algorithm that is best suited for the classification or prediction problem under investigation such as discriminate between groups of infants at high and low risk for autism using EEG data \cite{Elsabbagh_2009}).}
\label{fig:MVPA_schematic}
\end{figure*}

==> LaTeX_Figures/Process_FBD.tex <==
\usetikzlibrary{decorations.text}

\tikzstyle{block} = [rectangle, rounded corners, draw, text width=11.5cm, text badly centered, minimum height = 1 cm]
\tikzstyle{dotted_block} = [draw=black!30!white, line width=1pt, dash pattern=on 1pt off 4pt on 6pt off 4pt,
            inner ysep=6mm,inner xsep=4mm, rectangle, rounded corners ]
\tikzstyle{myarrows} = [ultra thick,->]

\newcommand{\arcarrow}[8]% inner radius, middle radius, outer radius, start angle, end angle, tip protusion angle, options, text
{   \pgfmathsetmacro{\rin}{#1}
    \pgfmathsetmacro{\rmid}{#2}
    \pgfmathsetmacro{\rout}{#3}
    \pgfmathsetmacro{\astart}{#4}
    \pgfmathsetmacro{\aend}{#5}
    \pgfmathsetmacro{\atip}{#6}
   \fill[#7] (\astart:\rin) arc (\astart:\aend:\rin) -- (\aend+\atip:\rmid) -- (\aend:\rout) arc (\aend:\astart:\rout) -- (\astart+\atip:\rmid) -- cycle;
    \path[ decoration={text along path, text={|\Huge| #8}, text align={center}, raise=-.5ex},decorate] ( \astart+\atip:\rmid) arc (\astart+\atip:\aend+\atip:\rmid);
}
\scalebox{.55}{
\begin{tikzpicture}[baseline]
    \fill[even odd rule,red!30] circle (4.2) circle (3.8);
    \foreach \x/\y in {0/Localisation, -120/Specialisation, -240/Parcellation} 
    {\arcarrow{3.4}{4}{4.6}{\x+20}{\x+120}{12}{blue!40,draw=blue!50!black,very thick}{\y}
    }
    % \node(n1)[dotted_block, minimum width = 11cm, minimum height = 10cm]{};
\end{tikzpicture}}

%\fill[#7] (\astart:\rin) arc (\astart:\aend:\rin) -- (\aend+\atip:\rmid) -- (\aend:\rout) arc (\aend:\astart:\rout) -- (\astart+\atip:\rmid) -- cycle;

==> LaTeX_Figures/RandomForest.tex <==
\tikzset{
  font=\Huge\bfseries,
  red arrow/.style={
    midway,red,sloped,fill, minimum height=3cm, single arrow, single arrow head extend=.5cm, single arrow head indent=.25cm,xscale=0.3,yscale=0.15,
    allow upside down
  },
%   black arrow/.style 2 args={-stealth, shorten >=#1, shorten <=#2},
%   black arrow/.style={thick, -{>[scale=2.5, width=6]}},
  tree box/.style={draw, rounded corners, inner sep=1em},
  node box/.style={white, draw=black, text=black, rectangle, rounded corners, minimum height = 2cm, minimum width = 4cm, inner sep=0.5cm},
}
\tikzstyle{black arrow} = [ultra thick,arrows={-Triangle[angle=90:10pt,black,fill=black]}]
% \begin{figure}
\scalebox{0.305}{
\begin{forest}
  for tree={l sep=3em, s sep=3em, anchor=center, inner sep=0.7em, draw, fill=yellow!50, circle, where level=2{no edge}{}}
  [
  Training Data, node box, alias=tdata, xshift = -1cm,
  [\begin{tabular}{c}
     Random Feature Selection and  \\
     Subset of Training Data  
  \end{tabular}, node box, alias=bagging, xshift = -1cm, above=4em
  [,red!70,draw=black,alias=a1[[,draw=black,alias=a2][]][,red!70,draw=black,edge label={node[above=1ex,red arrow]{}}[[][]][,red!70,draw=black,edge label={node[above=1ex,red arrow]{}}[,red!70,draw=black,edge label={node[below=1ex,red arrow]{}}][,alias=a3]]]]
  [,red!70,draw=black, alias=b1[,red!70, draw=black,edge label={node[below=1ex,red arrow]{}}[[,alias=b2][]][,red!70,draw=black,edge label={node[above=1ex,red arrow]{}}]][[][[][,alias=b3]]]]
  [~~$\dots$~,scale=2,no edge,fill=none,yshift=-4em, draw=none]
  [,red!70,draw=black,alias=c1[[,alias=c2][]][,red!70,draw=black,edge label={node[above=1ex,red arrow]{}}[,red!70,draw=black,edge label={node[above=1ex,red arrow]{}}[,alias=c3][,red!70,edge label={node[above=1ex,red arrow]{}}]][,draw=black,alias=c4]]]]
  ]
  \node[tree box, fit=(a1)(a2)(a3)](t1){};
  \node[tree box, fit=(b1)(b2)(b3)](t2){};
  \node[tree box, fit=(c1)(c2)(c3)(c4)](tn){};%yshift = -10.5cm, xshift = 9.5cm, scale = 1.5
  \node[below right=0.5em, inner sep=0pt] at (t1.north west) {Tree 1};
  \node[below right=0.5em, inner sep=0pt] at (t2.north west) {Tree 2};
  \node[below right=0.5em, inner sep=0pt] at (tn.north west) {Tree $n$};
  \path (t1.south west)--(tn.south east) node[below=4em of t2, node box] (mean) {Majority vote for classification};
  \node[below=3em of mean, node box] (pred) {Class Prediction};
  \draw[black arrow] (bagging) -| (t1.north);
  \draw[black arrow] (bagging.south) -- ([xshift=-.1cm]t2.north);
  \draw[black arrow] (bagging) -| (tn.north);
  \draw[black arrow] (t1.south) |- (mean);
  \draw[black arrow] (t2.south) -- (mean);
  \draw[black arrow] (tn.south) |- (mean);
  \draw[black arrow] (mean) -- (pred);
  \draw[black arrow] (tdata) -- (bagging.north);
\end{forest}}
% \caption{Random Forest (RF) are an ensemble of random decision trees i.e. RF classification mechanism generates \texttt{n} trees (classifiers) and aggregate their results. Since each tree is generated using randomly chosen features, and trained on a randomly chosen subset of training data, all trees in the RF have a different, uncorrelated classification path. \textcolor{red}{how is the path chosen?} Each tree predicts a label for the class independently, and the class that has the most votes is the predicted class. For most classification problems, the greater the number of trees in the RF, the better is the classification accuracy.}
% \label{fig:RF}
% \end{figure}

% how is the decision made in RF
% It is intuitively clear that for each decision that a tree (or a forest) makes there is a path (or paths) from the root of the tree to the leaf, consisting of a series of decisions, guarded by a particular feature, each of which contribute to the final predictions.
% A decision tree with M leaves divides the feature space into M regions Rm,1≤m≤M. In the classical definition (see e.g. Elements of Statistical Learning), the prediction function of a tree is then defined as f(x)=∑m=1McmI(x,Rm) where M is the number of leaves in the tree(i.e. regions in the feature space), Rm is a region in the feature space (corresponding to leaf m), cm is a constants corresponding to region m and finally I is the indicator function (returning 1 if x∈Rm, 0 otherwise). The value of cm is determined in the training phase of the tree, which in case of regression trees corresponds to the mean of the response variables of samples that belong to region Rm (or ratio(s) in case of a classification tree). The definition is concise and captures the meaning of tree: the decision function returns the value at the correct leaf of the tree. But it ignores the “operational” side of the decision tree, namely the path through the decision nodes and the information that is available there.

